Sleep Model -- A Sequence Model for Predicting the Next Sleep Stage

As sleep disorders are becoming more prevalent there is an urgent need to classify sleep stages in a less disturbing way.In particular, sleep-stage classification using simple sensors, such as single-channel electroencephalography (EEG), electrooculography (EOG), electromyography (EMG), or electrocardiography (ECG) has gained substantial interest. In this study, we proposed a sleep model that predicts the next sleep stage and used it to improve sleep classification accuracy. The sleep models were built using sleep-sequence data and employed either statistical $n$-gram or deep neural network-based models. We developed beam-search decoding to combine the information from the sensor and the sleep models. Furthermore, we evaluated the performance of the $n$-gram and long short-term memory (LSTM) recurrent neural network (RNN)-based sleep models and demonstrated the improvement of sleep-stage classification using an EOG sensor. The developed sleep models significantly improved the accuracy of sleep-stage classification, particularly in the absence of an EEG sensor.

==> tables/beamsearch-1column.tex <==
\begin{table}[t]
	\caption{The performance of the LSTM-RNN SLMs with 4 or 1 -channel signal models. The SLMs had 2 layers of LSTM with 1,024 hidden dimensions.}
	\centering\label{tab:beam-4ch-1ch}
	\begin{adjustbox}{width=0.99\columnwidth}
		{\setlength{\aboverulesep}{0.1em}
			\setlength{\belowrulesep}{0.15em}
			%\setlength{\tabcolsep}{3.5pt}
			\footnotesize
			\begin{tabular}{Sccrrrr}
				\multicolumn{6}{Sc}{\multirow{1}{*}{(a) 4-Channel Signal Model}}                         \\
				\cmidrule(){1-6}
				\multicolumn{1}{Sc}{\multirow{2}{*}{\shortstack{Sleep Stage                              \\Classification Model}}} &
				\multicolumn{1}{Sc}{\multirow{2}{*}{$\alpha$}}    &
				\multicolumn{2}{Sc}{\multirow{1}{*}{Valid.\ set}} &
				\multicolumn{2}{Sc}{\multirow{1}{*}{Test set}}                                           \\
				\cmidrule(lr){3-4}
				\cmidrule(lr){5-6}
				                                                  &       & Kappa & Acc.  & Kappa & Acc. \\
				\cmidrule(){1-6}
				Signal Model                                 &
				N/A                                               & 0.741 & 0.804 & 0.680 & 0.759        \\
				%2$\times$\phantom{0}256 & 
				%0.12 & \textbf{0.741} & \textbf{0.805} & \textbf{0.741} & %\textbf{0.805}  \\
				+ SLM Decording                                   &
				0.12                                              & 0.680 & 0.759 & 0.680 & 0.759        \\
				%4$\times$\phantom{0}256 & 
				%0.16 & 0.681 & 0.760 & 0.681 & 0.760  \\
				%4$\times$1024 & 
				%0.08 & 0.681 & 0.760 & 0.681 & 0.760  \\
				\midrule
				\\
				\multicolumn{6}{Sc}{\multirow{1}{*}{(b) 1-Channel Signal Model}}                         \\
				\cmidrule(){1-6}
				\multicolumn{1}{Sc}{\multirow{2}{*}{\shortstack{Sleep Stage                              \\Classification Model}}} &
				\multicolumn{1}{Sc}{\multirow{2}{*}{$\alpha$}}    &
				\multicolumn{2}{Sc}{\multirow{1}{*}{Valid.\ set}} &
				\multicolumn{2}{Sc}{\multirow{1}{*}{Test set}}                                           \\
				\cmidrule(lr){3-4}
				\cmidrule(lr){5-6}
				                                                  &       & Kappa & Acc.  & Kappa & Acc. \\
				\cmidrule(){1-6}
				Signal Model                                 &
				N/A                                               & 0.505 & 0.629 & 0.464 & 0.602        \\
				%2$\times$\phantom{0}256&
				%0.58 & 0.596 & 0.699 & 0.512 & 0.639\\
				+ SLM Decording                                   &
				0.42                                              & 0.596 & 0.698 & 0.519 & 0.644        \\
				%4$\times$\phantom{0}256 & 
				%0.54 & 0.593 & 0.696 & 0.520 & 0.644\\
				%4$\times$1024 &
				%0.60 & \textbf{0.602} & \textbf{0.703} & \textbf{0.523} & \textbf{0.647}\\
				\bottomrule
			\end{tabular}}
	\end{adjustbox}
\end{table}

==> tables/beamsearch-4ch.tex <==
\begin{table}[t]
\caption{The performance when the model with full PSG signal is decoded with the LSTM RNN sleep model. The beam width is 128.}\label{tab:beam-4ch}
\centering
\begin{adjustbox}{width=0.99\columnwidth}{
%\setlength{\aboverulesep}{0.25pt}
%\setlength{\belowrulesep}{0.25pt}
%\setlength{\tabcolsep}{3.5pt}
%\footnotesize
\begin{tabular}{Sccrrrr}
\toprule
\multicolumn{1}{Sc}{\multirow{1}{*}{LSTM RNN}} & 
\multirow{2}{*}{$\alpha$} &
\multicolumn{2}{Sc}{\multirow{1}{*}{Valid. set}} & 
\multicolumn{2}{Sc}{\multirow{1}{*}{Test set}} \\
Decoder & & Kappa & Acc. & Kappa & Acc. \\
\cmidrule(r{0.1em}){1-1} \cmidrule(l{0.1em}r{0.1em}){2-2} \cmidrule(l{0.1em}r{0.1em}){3-4} \cmidrule(l{0.1em}){5-6}
Signal Model & N/A & 0.741 & 0.804 & 0.680 & 0.759 \\
2$\times$\phantom{0}256 & 0.12 & \textbf{0.741} & \textbf{0.805} & \textbf{0.741} & \textbf{0.805} \\
2$\times$1024           & 0.12 & 0.680 & 0.759 & 0.680 & 0.759 \\
4$\times$\phantom{0}256 & 0.16 & 0.681 & 0.760 & 0.681 & 0.760 \\
4$\times$1024           & 0.08 & 0.681 & 0.760 & 0.681 & 0.760 \\
\bottomrule
\end{tabular}}
\end{adjustbox}
\end{table}

==> tables/beamsearch-eog.tex <==
\begin{table}[t]
\caption{The performance when the model with only EOG signal is decoded with the RNN sleep model. The beam width is 128.}
\label{tab:beam-1ch}
\centering
\begin{adjustbox}{width=0.99\columnwidth}{
%\setlength{\aboverulesep}{0.25pt}
%\setlength{\belowrulesep}{0.25pt}
%\setlength{\tabcolsep}{3.5pt}
%\footnotesize
\begin{tabular}{Sccrrrr}
\toprule
\multicolumn{1}{Sc}{\multirow{1}{*}{LSTM RNN}} & 
\multirow{2}{*}{$\alpha$} &
\multicolumn{2}{Sc}{\multirow{1}{*}{Valid. set}} & 
\multicolumn{2}{Sc}{\multirow{1}{*}{Test set}} \\
Decoder & & Kappa & Acc. & Kappa & Acc. \\
\cmidrule(r{0.1em}){1-1} \cmidrule(l{0.1em}r{0.1em}){2-2} \cmidrule(l{0.1em}r{0.1em}){3-4} \cmidrule(l{0.1em}){5-6}
Signal Model & N/A & 0.505 & 0.629 & 0.464 & 0.602 \\
2$\times$\phantom{0}256 & 0.58 & 0.596 & 0.699 & 0.512 & 0.639 \\
2$\times$1024           & 0.42 & 0.596 & 0.698 & 0.519 & 0.644 \\
4$\times$\phantom{0}256 & 0.54 & 0.593 & 0.696 & 0.520 & 0.644 \\
4$\times$1024           & 0.60 & \textbf{0.602} & \textbf{0.703} & \textbf{0.523} & \textbf{0.647} \\
\bottomrule
\end{tabular}}
\end{adjustbox}
\end{table}

==> tables/beamsearch_results.tex <==
\begin{table*}[t]
\caption{The performance when the signal model with full PSG signal or only EOG signal decoded with the LSTM RNN sleep models. The beam width is 128. The numbers in the first column represent (the number of layers) $\times$ (the size of the hidden dimension) for each SLM.}\label{tab:beam-4ch-1ch}
\centering
\begin{adjustbox}{width=0.8\textwidth}{
\setlength{\aboverulesep}{0.1em}
\setlength{\belowrulesep}{0.15em}
%\setlength{\tabcolsep}{3.5pt}
\footnotesize
\begin{tabular}{Sccrrrrcrrrr}
\toprule
\multicolumn{1}{Sc}{\multirow{3}{*}{\shortstack{\vspace{1.55em}\\LSTM-RNN\\Sleep Model}}} & 
\multicolumn{5}{Sc}{\multirow{1}{*}{4-Channel Signal Model}} &
\multicolumn{5}{Sc}{\multirow{1}{*}{1-Channel Signal Model}} \\
\cmidrule(lr){2-6}
\cmidrule(lr){7-11}
 & 
\multicolumn{1}{Sc}{\multirow{2}{*}{$\alpha$}} &
\multicolumn{2}{Sc}{\multirow{1}{*}{Valid. set}} & 
\multicolumn{2}{Sc}{\multirow{1}{*}{Test set}} & 
\multicolumn{1}{Sc}{\multirow{2}{*}{$\alpha$}} &
\multicolumn{2}{Sc}{\multirow{1}{*}{Valid. set}} & 
\multicolumn{2}{Sc}{\multirow{1}{*}{Test set}} \\
\cmidrule(lr){3-4}
\cmidrule(lr){5-6}
\cmidrule(lr){8-9}
\cmidrule(l){10-11}
 & & Kappa & Acc. & Kappa & Acc. & & Kappa & Acc. & Kappa & Acc. \\
\midrule
Signal Model & 
N/A & 0.741 & 0.804 & 0.680 & 0.759 & 
N/A & 0.505 & 0.629 & 0.464 & 0.602 \\
2$\times$\phantom{0}256 & 
0.12 & \textbf{0.741} & \textbf{0.805} & \textbf{0.741} & \textbf{0.805} &
0.58 & 0.596 & 0.699 & 0.512 & 0.639 \\
2$\times$1024 &
0.12 & 0.680 & 0.759 & 0.680 & 0.759 &
0.42 & 0.596 & 0.698 & 0.519 & 0.644 \\
4$\times$\phantom{0}256 & 
0.16 & 0.681 & 0.760 & 0.681 & 0.760 & 
0.54 & 0.593 & 0.696 & 0.520 & 0.644 \\
4$\times$1024 & 
0.08 & 0.681 & 0.760 & 0.681 & 0.760 &
0.60 & \textbf{0.602} & \textbf{0.703} & \textbf{0.523} & \textbf{0.647} \\
\bottomrule
\end{tabular}}
\end{adjustbox}
\end{table*}

==> tables/hmc-slm-perplexity.tex <==
\begin{table}[t]
\caption{The perplexity of LSTM RNN-based sleep models with HMC dataset. The number in the first row means (the number of layers) $\times$ (the size of the hidden dimension) of each SLM.}
\label{tab:hmc-ngram-lstm-pp}
\centering
\begin{adjustbox}{width=0.8\columnwidth}{
%\setlength{\aboverulesep}{0.25pt}
%\setlength{\belowrulesep}{0.25pt}
%\setlength{\tabcolsep}{3.5pt}
%\footnotesize
\begin{tabular}{Scrrrrr}
\toprule
%\multicolumn{1}{Sc}{N-gram} & 
%\multicolumn{1}{Sc}{2} &
%\multicolumn{1}{Sc}{3} &
%\multicolumn{1}{Sc}{4} &
%\multicolumn{1}{Sc}{5} &
%\multicolumn{1}{Sc}{6} \\
%\cmidrule(r{0.2em}){1-1} \cmidrule(l{0.2em}){2-6}
%Valid. set & 1.659 & 1.610 & 1.595 & 1.589 & 1.591 \\
%Test set  & 1.773 & 1.694 & 1.672 & 1.665 & 1.665 \\ \cmidrule(){1-6}
Model &
\multicolumn{1}{Sc}{\multirow{1}{*}{2$\times$256}} &
\multicolumn{1}{Sc}{\multirow{1}{*}{2$\times$1024}} &
\multicolumn{1}{Sc}{\multirow{1}{*}{4$\times$256}} &
\multicolumn{1}{Sc}{\multirow{1}{*}{4$\times$1024}} \\
\cmidrule(r{0.2em}){1-1} \cmidrule(l{0.2em}r{0.2em}){2-3} \cmidrule(l{0.2em}){4-5}
Valid. set & \textbf{1.546} & 1.547 & 1.547 & 1.548 \\
Test set  & 1.609 & \textbf{1.608} & 1.613 & 1.610 \\

\bottomrule
\end{tabular}}
\end{adjustbox}
\end{table}

==> tables/nchsdb_slm-perplexity.tex <==
%\begin{table}[t]
%\caption{\(NCHSDB sleep model perplexity\)}
%\label{tab:nchsdb-ngram-pp}
%\centering
%\begin{adjustbox}{width=0.99\columnwidth}{
%%\setlength{\aboverulesep}{0.25pt}
%%\setlength{\belowrulesep}{0.25pt}
%%\setlength{\tabcolsep}{3.5pt}
%%\footnotesize
%\begin{tabular}{Scrrrrrrrr}
%\toprule
%\multicolumn{1}{Sc}{N-gram} & 
%\multicolumn{1}{Sc}{2} &
%\multicolumn{1}{Sc}{3} &
%\multicolumn{1}{Sc}{4} &
%\multicolumn{1}{Sc}{5} &
%\multicolumn{1}{Sc}{6} &
%\multicolumn{1}{Sc}{7} &
%\multicolumn{1}{Sc}{8} &
%\multicolumn{1}{Sc}{9} &
%\\ \cmidrule(r{0.2em}){1-1} \cmidrule(l{0.2em}){2-9}
%Test set  &  &  &  &  &  &  & \\ \cmidrule(){1-6}
%LSTM & 
%\multicolumn{1}{Sc}{\multirow{3}{*}{2 x 512}} &
%\multicolumn{1}{Sc}{\multirow{2}{*}{2 x 1024}} \\
%Valid set & \multirow{3}{*}{1.547} & \multirow{2}{*}{1.547} \\
%Test set  & \multirow{3}{*}{1.609} & \multirow{2}{*}{1.608} \\
%
%\bottomrule
%\end{tabular}}
%\end{adjustbox}
%\end{table}

%%% LSTM Model %%%
\begin{table}[t]
\caption{The perplexity of LSTM RNN-based sleep models with NCHSDB. The number in the first row means (the number of layers) $\times$ (the size of the hidden dimension) of each SLM.}
\label{tab:nchsdb-lstm-pp}
\centering
\begin{adjustbox}{width=0.8\columnwidth}{
%\setlength{\aboverulesep}{0.25pt}
%\setlength{\belowrulesep}{0.25pt}
%\setlength{\tabcolsep}{3.5pt}
%\footnotesize
\begin{tabular}{Scrrrr}
\toprule
%\multicolumn{1}{Sc}{N-gram} & 
%\multicolumn{1}{Sc}{2} &
%\multicolumn{1}{Sc}{3} &
%\multicolumn{1}{Sc}{4} &
%\multicolumn{1}{Sc}{5} &
%\multicolumn{1}{Sc}{6} \\
%\cmidrule(r{0.2em}){1-1} \cmidrule(l{0.2em}){2-6}
%Valid. set & 1.659 & 1.610 & 1.595 & 1.589 & 1.591 \\
%Test set  & 1.773 & 1.694 & 1.672 & 1.665 & 1.665 \\ \cmidrule(){1-6}
%Layers & 
%\multicolumn{2}{Sc}{2} &
%\multicolumn{2}{Sc}{4} \\
%\cmidrule(r{0.2em}){1-1} \cmidrule(l{0.2em}r{0.2em}){2-3} %\cmidrule(l{0.2em}){4-5}
%Dim. 
%& \multicolumn{1}{Sc}{256} & \multicolumn{1}{Sc}{1024}
%& \multicolumn{1}{Sc}{256} & \multicolumn{1}{Sc}{1024} \\
Model &
\multicolumn{1}{Sc}{\multirow{1}{*}{2$\times$256}} &
\multicolumn{1}{Sc}{\multirow{1}{*}{2$\times$1024}} &
\multicolumn{1}{Sc}{\multirow{1}{*}{4$\times$256}} &
\multicolumn{1}{Sc}{\multirow{1}{*}{4$\times$1024}} \\
\cmidrule(r{0.2em}){1-1} \cmidrule(l{0.2em}r{0.2em}){2-3} \cmidrule(l{0.2em}){4-5}
Valid. set & \textbf{1.546} & 1.547 & 1.547 & 1.548 \\
Test set  & 1.609 & \textbf{1.608} & 1.613 & 1.610 \\
\bottomrule
\end{tabular}}
\end{adjustbox}
\end{table}
